GTNet:Guided Transformer Network for Detecting Human-Object Interactions

The human-object interaction (HOI) detection task refers to localizing humans, localizing objects, and predicting the interactions between each human-object pair. HOI is considered one of the fundamental steps in truly understanding complex visual scenes. For detecting HOI, it is important to utilize relative spatial configurations and object semantics to find salient spatial regions of images that highlight the interactions between human object pairs. This issue is addressed by the novel self-attention based guided transformer network, GTNet. GTNet encodes this spatial contextual information in human and object visual features via self-attention while achieving state of the art results on both the V-COCO and HICO-DET datasets. Code will be made available online.

==> content/1_abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
The human-object interaction (HOI) detection task refers to localizing humans, localizing objects, and predicting the interactions between each human-object pair. HOI is considered one of the fundamental steps in truly understanding complex visual scenes. For detecting HOI, it is important to utilize relative spatial configurations and object semantics to find salient spatial regions of images that highlight the interactions between human object pairs. This issue is addressed by the novel self-attention based guided transformer network, GTNet. GTNet encodes this spatial contextual information in human and object visual features via self-attention while achieving state of the art results on both the V-COCO~\cite{gupta2015visual} and HICO-DET~\cite{chao2018learning} datasets.   
\vspace{-0.4cm}
 \end{abstract}

 %GTNet, a  detect HOIs
  %GTNet, 
  %a 4\%-5\% improvement over previous 
  %Recent methods, however, fail to use prior information to its fullest potential to detect HOIs by
  
  %To truly understand complex visual scenes, machine vision requires detecting interactions among humans and objects, making human-object interaction (HOI) a significant part of intelligent systems.
  %Recent works try to leverage additional information (pose estimation for determining human actions, word embeddings for ideantifying the objects, etc.) derived from existing well-built neural networks as additional features to identify HOIs. Instead of just focusing on using more external cues, we propose a self-attention based guided network GTNet to determine subtle pairwise contextual information among each human and object pair. Inspired by the Transformer architecture in natural language processing (NLP), GTNet encodes contextual knowledge in  Additionally, a guiding mechanism based on external cues to guide the self-attention mechanism is developed. 


==> content/4_methodology.tex <==
\section{Technical Approach}
In this section, we introduce our proposed GTNet architecture for Human-Object interaction (HOI) detection. The task is, from an input image, to generate bounding boxes for all humans and objects while detecting the interactions among them (e.g. a person hitting a ball). Each human-object pair can have multiple interactions. Like most previous works, we will use a pre-trained object detector to detect humans and objects in the images. 

GTNet takes image features $\textbf{F}$  as input. For extracting features, we use standard object detection networks (e.g., resnet~\cite{he2016deep} and  efficientnet~\cite{tan2019efficientnet}).Along with image features, for each human and object our network takes bounding boxes $b_h$ and $b_o$ as inputs when there are $M\geq1$ humans and $N\geq1$ objects present in the image. As mentioned earlier, we use pre-trained obect detector to generate those bounding boxes. Our network will predict an interaction probability vector $\mathbf{p}_{HOI}$ for each human-object pair.

In the next sections, we will describe different components of our network.
%C
 %Consider a single image of size $c\times h\times w$ where $c,h,$ and $w$ are the number of channels, height and width of the image. For a given imFig. 3 details our take on the TX module.age, $\textbf{F}$ has a dimension of $C\times H\times W$ in the feature space. The relationship between $C,H,W$ and $c,h, W$ and  depends on the backbone network. 
 %Along with guiding the attention mechanism, we also utilize these relevant prior information to refine (Section~\ref{}) our naive features from the baseline module. 
%Our model architecture can be seen in Fig.~\ref{fig:model_architecture}.   
%\subsection{Problem Statement} \label{subsection:overview}
 

%where each row represents a human-object pair and each column represents interaction probability for a certain class of interaction. $p_{M}$ has a dimension of $T\times C$ where $T$ is the total number of possible human-object pairs ( $M\times N$) and $C$ is the number of interaction classes in consideration.
 %For the ease of explanation, in this section, we consider one single image with $M$ and $N$ number of humans and objects as input to the GTNet.
%We will not use any subscript to present the human-object pair for the ease of our explanation. Readers should assume all our equ.s are written for one single human-object pair. 
%Here, $M$ and $N$ are the total numbers of humans and objects present in the image.
\subsection{Baseline Module} \label{baseline}
Our baseline module extracts human and object feature vectors $\mathbf{f}_{H}$, and $\mathbf{f}_{O}$ from the input feature map $\mathbf{F}$. Following previous works~\cite{gao2018ican,ulutan2020vsgnet} we use region of interest pooling followed by a residual block and average pooling to extract these feature vectors. Moreover, we use the overall feature map $\mathbf{F}$ to get generalized context information by extracting feature vector $\mathbf{f}_{G}$ with average pooling. Recent works like VSGNet~\cite{ulutan2020vsgnet} use this feature vector as a representation of context, we argue that it is not rich enough to account for interaction specific contexts. This is why we propose the guided attention mechanism to encode task specific spatial contextual information.%\footnote{We use $\mathbf{F_{*}}$ to represent 3 dimensional feature map and $\mathbf{f_{*}}$ to represent one dimensional feature vector.}
%is similar to the visual branch of VGSNet~\cite{ulutan2020vsgnet}. %should I mention this?.It

To get a joint representation of these feature vectors, we concatenate and project them in the same space using a fully connected (FC) layer.
\begin{equation}
    \mathbf{f}_{B} = \mathbf{FC}_{B}(\mathbf{f}_{H}  \mathbin\Vert \mathbf{f}_{O}  \mathbin\Vert \mathbf{f}_{G})
\end{equation}
Here, $ \mathbin\Vert$ represents concatenation. 
This naive feature vector $\mathbf{f}_{B}$ is not adequate to detect all fine-grained HOIs. In the next sections, we will describe how to refine and couple visual features with human-object pairwise spatial contextual information.


\subsection{TX Module}\label{TX_Mod}
Vaswani et al.~\cite{vaswani2017attention} propose the Transformer network for processing sequential data in natural language processing (NLP). This network uses self attention~\cite{xu2015show} to find contextual dependence in sequential data. The original Transformer network introduces the concept of queries, keys, and values, which we adopt to the context of HOI detection. Fig.~\ref{fig:tx_unit} details our take on the TX module.  
%The naming scheme resembles the dataset retrieval task~\cite{}.
%To find each element's importance in sequential input data, the original Transformer network takes the input sequence features and projects them to queries, keys, and values. With scaled dot product attention, the network will generate an attention map from the queries and the keys to weigh the values for generating new features of the input sequence that are more aware of the context.

Queries are defined as the pairwise joint representation of human and object feature vectors ($\mathbf{f}_{H}$, $\mathbf{f}_{O}$). We get the pairwise representation by concatenation and projection.
\begin{equation}
    \mathbf{f}_{Q} = \mathbf{FC}_{T}(\mathbf{f}_{H}  \mathbin\Vert \mathbf{f}_{O})
\end{equation}
Here, $\mathbf{f}_{Q}$ is the query vector, and $ \mathbin\Vert$ represents concatenation operation. For a single human-object pair query vector has a length of $D$. 

Keys ($\mathbf{F}_{K}$) and values ($\mathbf{F}_{V}$) are generated from the input feature map ($\mathbf{F}$) by two separate $1\times1$ convolutions. 
\begin{flalign}
    &\mathbf{F}_{K} = \mathbf{conv}_{K}(\mathbf{F}) \\
    &\mathbf{F}_{V} = \mathbf{conv}_{V}(\mathbf{F})
\end{flalign}
    \begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth,height=2in]{Images/tx_unit.png}
\end{center}
\vspace{-0.4cm}
\caption{TX Module. From the input feature map, we generate key and value by $1\times 1$ convolutions.  With scaled dot-product attention, we produce an attention map for a particular human-object pair from the query and the key. This attention map is used to weigh the value to derive the contextually rich feature vector $\textbf{f}_{C}$. }
\vspace{-0.4cm}
\label{fig:tx_unit}
\end{figure}%\end{figure}
Here, $\mathbf{conv}_{K}$ and $\mathbf{conv}_{V}$ are two different $1\times1$ convolution operations. $\mathbf{F}_{K}$ and $\mathbf{F}_{V}$ can be thought of as two different representations of the input feature map. For a single image, both of them have the dimension of $D\times H\times W$. 
%Basically, the number of channels in $\mathbf{F}_{K}$ and $\mathbf{F}_{V}$ are equal to the length of each query vector. 

The query vectors are used to search keys, $\mathbf{F}_{K}$ to find pairwise contextual information. Imagine a person is talking on phone in an image. Our query vector representing the person and the phone pair finds the important region (i.e. close to the ear) in $\mathbf{F}_{K}$ to detect the interaction: talking on phone. 

This search process is done by scaled dot-product attention (equation~\ref{dot}). In each spatial location of $\mathbf{F}_{K}$, we take a channel-wise scaled dot-product with the query vector. Softmax is applied to present the important context for a particular query in probabilities.  

%TC
% Our TX Network will adapt the idea of queries, keys, and values to detect HOIs. We have taken a combined representation of human feature $f_H$ and object feature $f_O$ for each human-object pair by concatenation and projection to retrieve contextual information relevant to the interacting human-object pair. 
%TC 
% Here, $\mathbf{f_{Q}}$ will act as queries, $ \mathbin\Vert$ represents concatenation operation. From the input feature map, $\mathbf{F}$, we will generate keys ($\mathbf{F_{K}}$) and values ($\mathbf{F_{V}}$) by two $1 \times 1$ convolution operations. These two convolutional operations project the keys and values to different spaces. Also, we make sure that the queries' length is the same as the number of channels in keys and values.   

% Then we will apply scaled-dot product attention between $\mathbf{f_{Q}}$ and $\mathbf{F_{K}}$. The intuition is, with matrix-vector dot product, the self-attention mechanism will highlight certain regions spatially in $\mathbf{F_{K}}$, which is contextually important to detect HOIs for each of the queries. Scaling is done to normalize the multiplication. 
\begin{align}
    \mathbf{A} = \textbf{Softmax}(\frac{\mathbf{f}_{Q}\mathbf{F}_{K}^{T}}{\sqrt{\mathbf{D}}}) 
    \label{dot}
\end{align}
% $\mathbf{D_{re}}$ is the representation size equal to the length of $\mathbf{Q}$ and the number of channels in $\mathbf{K}$. (Check Supplementary Materials for more details.) 
For a particular query, $\mathbf{A}$ is the attention map where each element signifies the probability of that spatial location to be significant for detecting interactions. $\mathbf{A}$ has a dimension of $H\times W$ for each query vector. We use the attention map $\mathbf{A}$ to weigh $\mathbf{F}_{V}$ to get updated contextually rich query vectors. Following Transformer~\cite{vaswani2017attention}, we use fully connected layers with residual connections in this process.   
\begin{flalign}
    &\mathbf{f}_{C} = \sum\limits_{H,W}\mathbf{A}*\mathbf{F}_{V} \\ 
    &\mathbf{f}_{C}=LN(\mathbf{f}_{C}+\mathbf{f}_{Q}) \\
    &\mathbf{f}_{C}=LN(\mathbf{f}_{C}+\mathbf{FC}_{C}(\mathbf{f}_{C}))
\end{flalign}
Here, LN means layer norm. It is used to stabilize the operations and prevent overfitting during training. Also, $\mathbf{*}$ represents the Hadamard product between $\mathbf{A}$ and each channel of $\mathbf{F}_{V}$. The resultant weighted $\mathbf{F}_{V}$ was averaged over the spatial dimensions. $\mathbf{f}_{C}$ is the contextually enriched feature vector that will be used in the Inference Module.

We stack multiple TX Modules together to get better context representations in the updated queries like the original Transformer architecture~\cite{vaswani2017attention, girdhar2019video}.
%The intuition behind is with more heads and layers; we will get a more diverse representation of the query, key, and value. But there is a chance that with more heads or layers, our network will overfit. Balancing this trade-off, we empirically choose two heads and two layers combinations for V-COCO and two heads and three layers combinations in HICO-DET. 
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Images/guide_arch.png}
\end{center}
%\vspace{-0.4cm}
\caption{Guidance Module. Extracted human-object features are used to generate query vector $\mathbf{f}_{Q}$. We use relative spatial configuration and semantic word embeddings to derive spatial and semantic guidance vectors $\mathbf{f}_{S}$ and $\mathbf{f}_{W}$. With one to one element-wise multiplication, we encode spatial and semantic information to the query vector $\mathbf{f}_{Q}$. We overload symbol $\mathbf{f}_{Q}$ to represent both guided and not guided query vectors.}
%\caption{Importance of semantic priors in the guidance mechanism. Both of the human-object pairs have similar relative spatial relations. However, one person is holding a phone and the other person is holding corn. Semantic information about the objects along with the relative spatial configurations in the guidance mechanism will help to guide the query vector to encode rich spatial contextual information for separating hold and talking on the phone interactions. }
\label{fig:guide_arch}
\vspace{-0.4cm}
\end{figure}%\end{figure}

\subsection{Guidance Module} \label{guide}
As mentioned in many previous works~\cite{vaswani2017attention,girdhar2019video}, Transformer-like architectures do not perform well without location information embedded in queries. For action recognition, Girdhar et al.~\cite{girdhar2019video} embedded bounding box sizes and locations in the queries. HOI detection is a more subtle task as, along with the size of the humans and the objects, relative configurations among them are also important. To this end, we propose our guidance module that uses relative spatial configurations and semantic representations of humans and objects to guide the attention mechanism. Fig.~\ref{fig:guide_arch} details our take on the Guidance Module. 
\vspace{-0.1cm}
\paragraph{\textbf{Spatial Guidance:}}
Relative spatial configurations have proven to be very useful~\cite{chao2018learning,ulutan2020vsgnet,li2019transferable,gao2018ican} in detecting HOIs. Like existing works, we use a two-channel binary map with a dimension of $2\times 64\times 64$ to encode relative spatial configurations. For a human-object pair, the first channel is 1 in the location of the human-bounding box, whereas the second channel contains 1 in the location of the object bounding box. Everywhere else is zero in the binary map. Following~\cite{chao2018learning}, we use two convolutional layers along with average pooling and linear projection($FC_{S}$) to get a feature vector $\mathbf{f}_{S}$, representing the relative spatial configurations. We utilize $\mathbf{f}_{S}$ to guide the TX Module.
\vspace{-0.2cm}
\paragraph{\textbf{Semantic Guidance:}}%Most of the previous works use this feature vector directly in their networks. However, 
We argue that, although  $\mathbf{f}_{S}$ is a strong cue to detect HOIs, the information it conveys can be confusing without proper knowledge of the object. An example of this is shown in Fig.~\ref{fig:semantic_prior}. Correct semantic information about the objects can easily remove this confusion. That is why we combine semantic priors with spatial configurations. Instead of just using a look-up table for identifying each object, we use word embeddings (vector representation of words) from the publicly available Glove~\cite{pennington2014glove} model.  %As these embeddings are learned by parsing through a vast corpus, they are more expressive in conveying semantic information.like previousFig. 3 details our take on tFig. 3 details our take on the TX module.he TX module. works~\cite{peyre2019detecting, kim2020detecting}. 
For our specific case, every detected object by the object detector is represented with a vector. For example, phone and football are presented by two different vectors. We express humans with one fixed vector.
% %These word embeddings are not expensive because we already know the identity of each object from the object detector. As a result, we do not need to run or fine tune any network to generate these embedding vectors. 
After concatenation of these human and object word embedding vectors together we get a combined feature vector $\mathbf{f}_{W}$ with linear projection ($FC_{W}$). Along with $\mathbf{f}_{S}$, we utilize $\mathbf{f}_{W}$ in the guiding mechanism. 
%\vspace{-0.1cm}
\paragraph{\textbf{Guidance Mechanism:}}The information present in $\mathbf{f}_{S}$ and $\mathbf{f}_{W}$ is used to guide the queries sent to the TX Module. Guiding here refers to encoding relative spatial configurations and semantic priors to the queries before feeding them to the TX Module so that our updated queries can be both location and context-aware. We achieve this encoding by taking the element-wise product among the spatial, semantic ,and the query vectors.
\begin{align}
    \mathbf{f}_{Q} = {\mathbf{f}_{Q}\circ \mathbf{f}_{S}\circ \mathbf{f}_{W}} 
    \label{eq:HADA}
\end{align}
Here, $\circ$ represents element wise dot product. We feed the guided query vector $f_{Q}$ to the TX Module. %We can derive the used prior information directly from the pre-trained object detector. As a result, these priors do not add any additional cost to the existing network.
\subsection{Inference Module} \label{fuse}
According to~\cite{yosinski2014transferable}, fusing features from different layers of a neural network increases the expressive capability of the features. Therefore, we fuse features from our Baseline Module with the TX Module. Moreover, we refine the naive visual features $\mathbf{f}_{B}$ in the same way as equ. ~\ref{eq:HADA}.
\begin{align}
    \mathbf{f}_{BR} = {\mathbf{f}_{B}\circ \mathbf{f}_{S}\circ \mathbf{f}_{W}} 
    \label{eq:HADA2}
\end{align}
We concatenate $\mathbf{f}_{B}$, $\mathbf{f}_{BR}$, $\mathbf{f}_{C}$ together to increase the diversity in the final feature representation. With fully connected layers we make class-wise predictions for each human-object pair over this concatenated feature. Following~\cite{li2019transferable, ulutan2020vsgnet}, we also generate an interaction proposal score, $\mathbf{b}_{I}$ using the baseline features for each human-object pair. This score represents the probability of interactions between a human-object pair irrespective of the class. 
%As mentioned in Section ~\ref{subsection:overview}, for a single input image with total $T$ number of human-object pairs and $C$ number of classes, the output of GTNet would be:

\begin{flalign}
    &\mathbf{p}_{I} = \sigma(\mathbf{FC}_{P}(\mathbf{f}_{B}  \mathbin\Vert \mathbf{f}_{BR}  \mathbin\Vert \mathbf{f}_{C})) \\ 
    &\mathbf{b}_{I}= \sigma(\mathbf{FC}_{P_{B}}(\mathbf{f}_{B}  \mathbin\Vert \mathbf{f}_{BR})) 
    %&\mathbf{p_{M}}= \mathbf{p_{I}}\times \mathbf{b_{I}}
\end{flalign}
Here, $\sigma$ represents a sigmoid non-linearity. For each human-object pair, we achieve our final predictions by multiplying these two individual predictions. 
\begin{align}
\mathbf{p}_{HOI}= \mathbf{p}_{I}\times \mathbf{b}_{I}
\label{final_pred}
\end{align}
$\mathbf{p}_{HOI}$ has a length equal to the number of classes in considerations. 
 %$\mathbf{p_{I}}$, $\mathbf{b_{I}}$, $\mathbf{p_{M}}$ have dimensions of $T\times C$, $T\times 1$, $T\times C$    
 \begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth,height=4.4cm]{Images/guide.png}
\end{center}
\vspace{-0.4cm}
%\caption{Guidance Module. Extracted human-object features are used to generate query vector $\mathbf{f}_{Q}$. We use relative spatial configuration and semantic word embeddings to derive spatial and semantic guidance vectors $\mathbf{f}_{S}$ and $f_{W}$. With one to one element-wise multiplication, we encode spatial and semantic information to the query vector $\mathbf{f}_{Q}$. We overload symbol $\mathbf{f}_{Q}$ to represent both guided and not guided query vectors.}
\caption{Importance of semantic priors in the guidance mechanism. Both of the human-object pairs have similar relative spatial relations. However, one person is holding a phone and the other person is holding corn. Semantic information about the objects along with the relative spatial configurations in the guidance mechanism will help to guide the query vector to encode rich spatial contextual information for separating hold and talking on the phone interactions. }
\label{fig:semantic_prior}
\vspace{-0.4cm}
\end{figure}%\end{figure}

==> content/old_results.tex <==
\begin{table}[]
%\hskip0.3cm
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}l@{}}Baseline \\ Module\end{tabular} & \begin{tabular}[c]{@{}l@{}}TX \\ Module\end{tabular} & \begin{tabular}[c]{@{}l@{}}Spatial \\ guidance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Semantic \\ guidance\end{tabular} & Scenario 1            \\ \hline
\cmark                                                     & \xmark                                               & \xmark                                                      & \xmark                                                       & 51.6          \\
\cmark                                                     & \cmark                                               & \xmark                                                      & \xmark                                                       & 52.0          \\
\cmark                                                     & \cmark                                               & \cmark                                                      & \xmark                                                       & 52.7          \\
\cmark                                                     & \cmark                                               & \xmark                                                      & \cmark                                                       & 55.9          \\ \hline
\cmark                                                     & \cmark                                               & \cmark                                                     & \cmark                                                       & \textbf{56.4} \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.08cm}
\caption{Dissection of different modules of GTNet in V-COCO test set. Each row represents a different experimental settings. (\cmark) indicates a module is included in the experiment and (\xmark) indicates a module is excluded from the experiment. GTNet achieves state of the art performance with the guidance mechanism. It is interesting to observe that, in the same dataset, semantic guidance performs better than spatial guidance when tested independently.}
%TX Module improves the baseline a little without the Guidance Module.}
\label{tab:diff_mod}
\vspace{-0.2cm}
\end{table}


\begin{table}[]
%\hskip0.3cm
\begin{adjustbox}{width=\columnwidth,center}
%\centering
\begin{tabular}{|l|l|}
\hline
                            & Scenario 1  \\ \hline
Baseline Module w/o Data Augmentation      & 49.6 \\
Baseline Module  w  Data Augmentation     & 51.6 \\ \hline
GTNet w/o Data Augmentation &     55.0 \\
GTNet w/ Data Augmentation   & 56.4 \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.08cm}
\caption{Strength of our data augmentation pipeline in V-COCO test set. Our Baseline Module achieves superior performance with data augmentation. Overall, GTNet performs better with the augmentation.}
\vspace{-0.5cm}
\label{tab:data_aug}
\end{table}

\begin{table}[]
%\hskip0.3cm
%\begin{adjustbox}{width=\columnwidth}
\centering
\begin{tabular}{|l|r|r|}

\hline
Method & \multicolumn{1}{l|}{Scenario 1} & \multicolumn{1}{l|}{Scenario 2} \\ \hline
VSGNet~\cite{ulutan2020vsgnet} & 67.4                            & 69.9                            \\
GTNet  & \textbf{72.6}                   & \textbf{74.6}                   \\ \hline
\end{tabular}
%\end{adjustbox}
\vspace{0.1cm}
\caption{Performance of GTNet in oracle object detector settings. Our performance improvement is better than the relavent attention based work VSGNet~\cite{ulutan2020vsgnet}.}
\label{tab:oracle}
\vspace{-0.4cm}
\end{table}





\begin{table}[]
%\hskip0.3cm
%\begin{adjustbox}{width=\columnwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
Number of  Channels & \multicolumn{1}{l|}{Scenario 1} & \multicolumn{1}{l|}{Scenario 2} \\ \hline
64                  & 57.21                           & 61.1                            \\
128                 & 57.46                           & 61.6                            \\
256                 & 57.48                           & 61.25                           \\
512                 & 58.29                           & 61.85                           \\ \hline
\end{tabular}
%\end{adjustbox}
\vspace{0.1cm}
\caption{Performance of GTNet with different number of channels for key and value.}
\label{tab:oracle}
\vspace{-0.4cm}
\end{table}

==> content/tables.tex <==
\begin{table*}[]
%\hskip1.0cm
\begin{adjustbox}{width=\columnwidth*2,center}
\centering
\begin{tabular}{|l|l|c|c|c|c|c|c|}
\hline
Method                                & Feature Backbone & Full(def) & Rare(def) & None-Rare(def) & Full(ko) & Rare(ko) & None-Rare(ko) \\ \hline
UnionDet~\cite{kim2020detecting}      & ResNet50-FPN     & 17.58     & 11.72     & 19.33          & 19.76    & 14.68    & 21.27         \\
IPNet~\cite{wang2020learning}         & Hourglass-104    & 19.56     & 12.79     & 21.58          & 22.05    & 15.77    & 23.92         \\
PPDM~\cite{liao2020ppdm}              & Hourglass-104    & 21.1      & 14.46     & 23.09          & -        & -        & -             \\
Functional~\cite{bansal2020detecting} & ResNet-101       & 21.96     & 16.43     & 23.62          & -        & -        & -             \\
Hou et al.~\cite{hou2020visual}       & ResNet-50        & 23.63     & 17.21     & 25.55          & 25.98    & 19.12    & 28.03         \\
ConsNet~\cite{liu2020consnet}         & ResNet-50        & 24.39     & 17.1      & 26.56          & -        & -        & -             \\
DRG~\cite{gao2020drg}                 & ResNet50-FPN     & 24.53     & 19.47     & 26.04          & 27.98    & 23.11    & 29.43         \\
IDN~\cite{IDN}                        & ResNet-50        & 26.29     & \textbf{22.61}     & 27.39          & 28.24    & \textbf{24.47}    & 29.37         \\ \hline
GTNet                                 & ResNet-50        & 26.78     & 21.02     & 28.5           & 28.80     & 22.19    & 30.77         \\
GTNet                                 & ResNet-152       & \textbf{28.30}      & 22.02     & \textbf{30.16}          & \textbf{30.31}    & 23.63    & \textbf{32.30}          \\ \hline \hline
iCAN~\cite{gao2018ican}                                  & ResNet-50        & 33.38     & 21.43     & 36.95          & -        & -        & -             \\
Li et al.~\cite{li2019transferable}                       & ResNet-50        & 34.26     & 22.9      & 37.65          & -        & -        & -             \\
Peyre et al.~\cite{peyre2019detecting}                               & ResNet-50-FPN    & 34.35     & 27.57     & 36.38          & -        & -        & -             \\
IDN~\cite{IDN}                                   & ResNet-50        & 43.98     & \textbf{40.27}     & 45.09          & -        & -        & -             \\ \hline
GTNet                                 & ResNet-50        & 44.71     & 33.8      & 47.97          & 44.71    & 33.8     & 47.97         \\
GTNet                                 & ResNet-152       & \textbf{46.78}     & 34.87     & \textbf{50.34}          & \textbf{46.78}    & \textbf{34.87}    & \textbf{50.34}         \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.08cm}
\caption{Performance comparisons in the HICO-DET~\cite{chao2018learning} test set. . }
\label{tab:hico-det_t}
\vspace{-0.4cm}
\end{table*}

%  In full setting all test images are used for evaluation. In rare and non-rare setting two smaller separate sets of test images are used for evaluation. These sets are created on the basis of the number of training samples
\begin{table}[]
%\hskip1.0cm
\begin{adjustbox}{width=\columnwidth,center}
\centering
\begin{tabular}{|l|l|c|c|}
\hline
Method                                   & Feature Backbone & Scenario 1    & Scenario 2    \\ \hline
T. Wang et. al.~\cite{wang2019deep}      & ResNet-50        & 47.3          & -             \\
DRG~\cite{gao2020drg}                    & ResNet50-FPN     & 51.0          & -             \\
VSGNet~\cite{ulutan2020vsgnet}           & ResNet - 152     & 51.8          & 57.0          \\
Wan et al.~\cite{wan2019pose}            & ResNet50-FPN     & 52.0          & -             \\
Zhong et al.~\cite{zhong2020polysemy}    & ResNet - 152     & 52.6          & -             \\
H. Wang et.al.~\cite{wang2020contextual} & ResNet50-FPN     & 52.7          & -             \\
Kim et al.~\cite{kim2020detecting}       & ResNet - 152     & 53.0          & -             \\
Liu et al.~\cite{liuamplifying}          & ResNet-50        & 53.1          & -             \\
ConsNet~\cite{liu2020consnet}                       & ResNet-50        & 53.2          & -             \\
IDN~\cite{IDN}                           & ResNet-50        & 53.3          & 60.3          \\
OSGNet~\cite{zhang2020improved}                           & ResNet-152        & 53.4          &    -      \\
Sun et al.~\cite{sun2020human}           & ResNet - 101     & 55.2          & -             \\
DIRV~\cite{fang2020dirv}                 & EfficientDet-d3  & 56.1          & -             \\ \hline
GTNet                                    & ResNet-50        & 56.2          & 60.1          \\
\textbf{GTNet}                           & ResNet-152       & \textbf{58.3} & \textbf{61.9} \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.08cm}
\caption{Performance comparisons in the  V-COCO~\cite{gupta2015visual} test set. Many current works do not report their models' performance in Scenario 2.}
\label{tab:v-coco}
\vspace{-0.4cm}
\end{table}

\begin{table*}[]
%\hskip1.0cm
\begin{adjustbox}{width=\columnwidth*2,center}
\centering
\begin{tabular}{|l|l|c|c|c|c|c|c|}
\hline
Method                                & Feature Backbone       & Full(def) & Rare(def) & None-Rare(def) & Full(ko) & Rare(ko) & None-Rare(ko) \\ \hline
VSGNet                                & ResNet-152             & 19.8      & 16.05     & 20.91          & -        & -        & -             \\
FCMNet                                & ResNet-50              & 20.41     & 17.34     & 21.56          & 22.04    & 18.97    & 23.12         \\
ACP                                   & ResNet-152             & 20.59     & 15.92     & 21.98          & -        & -        & -             \\
PD-Net                                & ResNet-152             & 20.81     & 15.9      & 22.28          & 24.78    & 18.88    & 26.54         \\
DJ-RN                                 & Resnet-50 and PointNet & 21.34     & 18.53     & 22.18          & 23.69    & 20.64    & 24.6          \\
OSGNet                                & ResNet-152             & 21.4      & 18.12     & 22.38          & -        & -        & -             \\
DIRV                                  & EfficientDet-d3        & 21.78     & 16.38     & 23.39          & 25.52    & 20.84    & 26.92         \\
ConsNet                               & ResNet-50              & 22.15     & 17.12     & \textbf{23.65}          & -        & -        & -             \\
IDN                                   & ResNet-50              & \textbf{23.36}     & \textbf{22.47}     & 23.63          & \textbf{26.43}    & \textbf{25.01}    & \textbf{26.85}         \\ \hline 
GTNet                                 & ResNet-50              & 20.87     & 17.51     & 21.88          & 23.72    & 19.56    & 24.97         \\ 
GTNet                                 & ResNet-152             & 22.28     & 17.87     & 23.6           & 25.24    & 20.66    & 26.61         \\ \hline \hline

\end{tabular}
\end{adjustbox}
\vspace{0.08cm}
\caption{Performance comparisons in the HICO-DET~\cite{chao2018learning} test set.  }
\label{tab:hico-det_f}
\vspace{-0.4cm}
\end{table*}
%  In full setting all test images are used for evaluation. In rare and non-rare setting two smaller separate sets of test images are used for evaluation. These sets are created on the basis of the number of training samples.





\begin{table}[]
%\hskip0.3cm
%\begin{adjustbox}{width=\columnwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
Number of  Channels & \multicolumn{1}{l|}{Scenario 1} & \multicolumn{1}{l|}{Scenario 2} \\ \hline
64                  & 57.21                           & 61.1                            \\
128                 & 57.46                           & 61.6                            \\
256                 & 57.48                           & 61.25                           \\
512                 & 58.29                           & 61.85                           \\ \hline
\end{tabular}
%\end{adjustbox}
\vspace{0.1cm}
\caption{Performance of GTNet with different number of channels for key and value.}
\label{tab:oracle}
\vspace{-0.4cm}
\end{table}

